AID-Purifier: A Light Auxiliary Network for Boosting Adversarial Defense

We propose an AID-purifier that can boost the robustness of adversarially-trained networks by purifying their inputs. AID-purifier is an auxiliary network that works as an add-on to an already trained main classifier. To keep it computationally light, it is trained as a discriminator with a binary cross-entropy loss. To obtain additionally useful information from the adversarial examples, the architecture design is closely related to information maximization principles where two layers of the main classification network are piped to the auxiliary network. To assist the iterative optimization procedure of purification, the auxiliary network is trained with AVmixup. AID-purifier can be used together with other purifiers such as PixelDefend for an extra enhancement. The overall results indicate that the best performing adversarially-trained networks can be enhanced by the best performing purification networks, where AID-purifier is a competitive candidate that is light and robust.

==> TEX/50_discussion.tex <==
\section{Discussions}
\label{sec:discussions}

\subsection{Adversarial purifiers as performance boosters}
\label{sec:booster}
In Section~\ref{sec:experiment_non_purification}, it was shown that AID-Purifier and PixelDefend can be highly useful as add-on defenders that can be used in addition to a high-performance defender such as Madry, Zhang, and Lee. When the computational overhead of purification is of concern, AID-Purifier alone can be used as a computationally light add-on. When the computational overhead of purification is not of concern, both of AID-Purifier and PixelDefend can be used together for an extra improvement in robust accuracy. 
% The extra improvement is due to the diversity between the two purifiers. PixelDefend's purification is based on the distribution $p_{data}(x)$ that is learned by PixelCNN. AID-Purifier's purification is based on the distributions $p_{clean}$ and $p_{adv}$ that are learned by the discriminator. While PixelDefend attempts to purify an example by pushing it to a high $p_{data}(x)$ region, AID-Purifier is more adventurous because it is willing to utilize out-of-distribution regions as well. The diversity between the two purifiers create a room for synergy. 

Considering the high performance of latest adversarially-trained models, it might be fair to assume that an adversarially-trained model should be always used as the base model while one or more purifiers could be used to boost its performance. 
% To investigate if AID-Purifier can create a positive synergy with purifiers other than PixelDefend, we have carried out an extra experiment. In Appendix~\ref{sec:comparison_nrp}, NRP~\cite{naseer2020self} instead of PixelDefend is used to create a table in the same form as Table~\ref{tab:comparison_w_adv_training}. NRP is a type of adversarial purifier, that trains a conditional GAN to learn an optimal input processing function that enhances model robustness.
% For NRP, the results in Table~\ref{tab:comparison_w_adv_training_appendix} of Appendix~\ref{sec:comparison_nrp} are similar to PixelDefend's results - AID-Purifier and NRP can create positive synergies. For the case of Defense-GAN, we have shown in Appendix~\ref{sec:stand-alone_add-on_appendix} that it can have negative effects for CIFAR-10, CIFAR-100, and TinyImageNet. In any case, we have tried using AID-Purifier together with Defense-GAN, and we have found that the loss by Defense-GAN can be mitigated by AID-Purifier as shown in Appendix~\ref{sec:comparison_dfgan}. 

Even though we have considered only adversarially-trained models as the base models to improve, the base model does not need to be limited in such a way. As long as a purifier is light in computation and attachable to frozen networks, it can be used as an add-on to boost \textit{any} adversarial defense network. 
% For the case of PixelDefend and NRP, the results in Table~\ref{tab:comparison_w_adv_training} and Table~\ref{tab:comparison_w_adv_training_appendix} can be carefully examined to confirm that AID-Purifier can positively improve stand-alone defense of PixelDefend or NRP. This confirms that it is not necessary for an adversarially-trained network to be the base model, and a stand-along purifier can be the base model to be improved. 
PixelDefend and NRP, however, are also auxiliary purifiers and perhaps they should not be considered as a base model. In general, it remains as a future work to answer if adversarial purifiers should be always included as the last step add-on. 


\vspace*{-.2cm}
\subsection{Limitations and additional investigations}
\label{sec:limitation} 
In contrast to the mainstream purification methods, AID-Purifier does not aim to modify an adversarial image to a clean image. Our method allows $x_{pur}$ to be moved to out-of-distribution regions, and it can be confirmed from $x_{pur}$ in Figure~\ref{fig:our_method}. The image is a real example of $x_{pur}$ that was created by AID-Purifier. 

% \citet{tramer2020adaptive} found that many combined defenses result in lower robustness than adversarial training alone, and a strong adaptive attack can be used to reveal the problem. In our study, we have performed auxiliary-aware attack as a strong adaptive attack and showed that the purification add-on is robust to the attack. Furthermore, we have investigated the influence of attack hyperparameters, attack epsilon, and the number of attack iterations for PGD attack as shown in Appendix~\ref{sec:sensitivity_appendix_att_hp}, and found that AID-Purifier can boost the performance for all the cases that were studied. Nonetheless, there might be other strong adaptive attacks that we might have missed to investigate.  

% We additionally investigate the sensitivities of the attack method, the defense epsilon, and the number of iterations for training discriminator. The results can be found in Appendix~\ref{sec:sensitivity_appendix_att_for_D} and~\ref{sec:sensitivity_appendix_def_eps_iter}. 


% \subsection{Negative societal impacts}
% \label{sec:Negativesocietalimpacts} 
% Our study may increase the understanding of the attackers who aim to attack the deep learning systems. However, we believe our study will contribute to the knowledge of the research community and be used in positive directions. 


==> TEX/9910_introduction_bu.tex <==
\section{Introduction}
\label{sec:introduction}

% Editage 수정본
Deep neural networks are vulnerable to adversarial examples generated by adding imperceptible adversarial perturbations to the original examples~\cite{szegedy2013intriguing}. 
To address this problem, various adversarial defense schemes have been proposed, where a vast majority of them can be grouped into three categories. 
%
The first category is \textit{gradient masking}~\cite{Xiao2020Enhancing, athalye2018obfuscated}, where the gradient of the classifier is hidden or obfuscated to obstruct gradient-based adversarial attacks.   
%
The second category is \textit{adversarial training}~\cite{madry2017towards, pmlr-v97-zhang19p,lee2020adversarial}, where the training dataset is augmented with adversarial examples. 
%
The third category is \textit{adversarial purification}~\cite{samangouei2018defensegan, song2018pixeldefend, meng2017magnet, shi2021online}, where a purification procedure is applied before the input example is passed to the main classifier. 

Although gradient masking is an effective method against gradient-based adversarial attacks, a few critical limitations have been identified. \citet{athalye2018obfuscated} showed that defenses relying on obfuscated gradients can be circumvented. In particular, they developed attack techniques for the three types of obfuscated gradients they discovered. \citet{papernot2017practical} demonstrated that black-box attacks often perform better than white-box attacks when the defense is a gradient-based method.
Compared to gradient masking, adversarial training turned out to be much more robust against known adversarial attacks. Robustness is due to the inherent improvement in generalization over adversarial examples, and adversarial training is considered to be the most effective adversarial defense as of today. \citet{madry2017towards} exploited a projected gradient descent (PGD) attack to augment the training dataset, \citet{pmlr-v97-zhang19p} minimized the trade-off between the natural and robust errors when training, and \citet{lee2020adversarial} suggested a soft-labeled data augmentation, called AVmixup, for improving adversarially robust generalization.


\begin{figure*}[t]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{m{5cm}m{5cm}m{5cm}m{5cm}}
\centering
 \includegraphics[width=0.6\linewidth]{FIGURE/1_a.jpg}
& \includegraphics[width=0.6\linewidth]{FIGURE/1_b.jpg}
& \includegraphics[width=0.6\linewidth]{FIGURE/1_c.jpg}
& \includegraphics[width=0.6\linewidth]{FIGURE/1_d.jpg} \\
\\
\multicolumn{1}{c}{\includegraphics[width=0.15\linewidth]{FIGURE/2_a.jpg}} 
& \multicolumn{2}{c}{\includegraphics[width=0.15\linewidth]{FIGURE/2_b.jpg}}  
& \multicolumn{1}{c}{\includegraphics[width=0.15\linewidth]{FIGURE/2_c.jpg}}  \\
\multicolumn{1}{c}{(a) Denoising Purifier} &
\multicolumn{1}{c}{(b) Generative Purifier} &
\multicolumn{1}{c}{(c) Generative Purifier} &
\multicolumn{1}{c}{(d) SSL-based Purifier} \\
\multicolumn{1}{c}{(MagNet~\cite{meng2017magnet})} &
\multicolumn{1}{c}{(Defense-GAN~\cite{samangouei2018defensegan})} &
\multicolumn{1}{c}{(PixelDefend~\cite{song2018pixeldefend})} &
\multicolumn{1}{c}{(SOAP~\cite{shi2021online})} \\

\end{tabular}
}
\caption{Summary of four existing purifiers. The upper diagrams show algorithm overviews. We denote main classification network as $C$, auxiliary network as Aux, network with frozen weights in gray, and network to be trained in green. The lower diagrams show the conceptual relationships between $x_{clean}$, $x_{adv}$, and $x_{pur}$. 
}
% \end{center}
\vspace*{-0.5cm}
\label{fig:purification_concept}
\end{figure*}


In this study, we focus on the third category, adversarial purification. Our objective is to develop a computationally light and easily attachable purifier such that it can be utilized as an add-on. Specifically, we show that we can boost the performance of \citet{madry2017towards,pmlr-v97-zhang19p}, and \citet{lee2020adversarial} with a light auxiliary network named \textit{AID-Purifier}. AID-Purifier utilizes \textbf{A}Vmixup, \textbf{I}nformation maximization principles, and \textbf{D}iscriminative task as the underlying foundations.
Before describing AID-Purifier, we first summarize previous works on adversarial purification methods. 





Adversarial purification modifies input examples to increase adversarial robustness, and four well-known purification methods are shown in Figure~\ref{fig:purification_concept}. 
In (a), a \textit{denoising purifier}, MagNet~\cite{meng2017magnet}, is shown. 
It uses an auto-encoder, called a reformer, as an auxiliary network for denoising adversarial perturbations. 
It is a straightforward approach in that its objective is to return an adversarial example $x_{adv}$ back to the original clean example $x_{clean}$. 
The resulting network as a whole, however, becomes just another feedforward network that is vulnerable to auxiliary-aware white-box attacks~\cite{tramer2020adaptive}. In (b), a \textit{generative purifier}, Defense-GAN~\cite{samangouei2018defensegan}, is shown. It uses an independently trained GAN to project $x_{adv}$ to a purified example $x_{pur}$ that belongs to the clean distribution $p_{data}(x)$. Unlike denoising purifiers, there is no known auxiliary-aware attack that is effective. Defense-GAN, however, is not easy to train, and its performance is worse than that of another well-known generative purifier. 
In (c), another generative purifier, PixelDefend~\cite{song2018pixeldefend}, is shown. Its performance is much better than that of Defense-GAN, especially for more complex datasets. PixelDefend, however, is computationally heavy owing to its pixel-wise operation. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[b!]
\begin{center}
\vspace*{-0.7cm}
\includegraphics[width=0.9\columnwidth]{FIGURE/ours_.jpg}
\caption{Algorithm overview and conceptual relationship of AID-Purifier. $D$ is the discriminator network.}
\label{fig:our_method}
\end{center}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
In (d), a \textit{self-supervised-learning-based purifier}, SOAP~\cite{shi2021online}, is shown. It is similar to generative purifiers, but it projects $x_{adv}$ to a purified example $x_{pur}$ belonging to a low $\mathcal{L}_{SSL}$ region. SOAP yields competitive robust accuracy against state-of-the-art adversarial training and purification methods, but it needs to be jointly trained with the main classifier $C$. Of the four purification methods in Figure~\ref{fig:purification_concept}, SOAP is the only one that requires joint training and thus cannot be used as an add-on. 




We herein propose a \textit{discriminative purifier} named AID-Purifier. To the best of our knowledge, this is the first successful purification method based on a discrimination task. AID-Purifier uses an auxiliary discriminator network $D$ to project $x_{adv}$ to a purified example $x_{pur}$ that belongs to a low $p_{adv}(x)$ region. Compared to the four methods in Figure~\ref{fig:purification_concept}, AID-Purifier is distinct because it has all the advantages of the four methods. 
Unlike denoising purifiers, it is robust against auxiliary-aware attacks. Unlike generative purifiers, it requires light computation and is easy to train. Unlike SOAP, it is an add-on that can be attached to any frozen state-of-the-art network. AID-Purifier is an effective stand-alone defense method; however, it can also create synergies with adversarially-trained networks or other purifier networks such as PixelDefend. For all experiments we performed, AID-Purifier was able to boost the robustness of state-of-the-art adversarial training and purification methods. 






==> TEX/9920_related_works_bu.tex <==
\section{Related Works}
\label{sec:Related Works}


\subsection{Detecting adversarial examples with an auxiliary network}
\label{sec:background:adversarialdetector}
For humans, it is difficult to tell the difference between a clean example and its adversarial example. The difference, however, can be detected well by training a binary classification network~\cite{gong2017adversarial,metzen2017detecting}. A standard binary cross-entropy (BCE) loss can be used for training, where the loss is interpreted as the probability of an adversarial example. 
%
\citet{gong2017adversarial} demonstrated that an independent and simple adversarial detector can be trained using a labeled dataset comprising clean and adversarial examples. Furthermore, they showed that the detector is robust to a second-round adversarial attack, similar to the auxiliary-aware attack in our work.
%
\citet{metzen2017detecting} considered a small subnetwork and concluded that a reliable adversarial detector could be trained. The subnetwork is essentially an auxiliary network attached to the main classification network $C(x)$, and it utilizes one of the hidden layers' representation as the input. 
% 
Even though such detectors clearly prove that the difference between $p_{clean}(x)$ and $p_{adv}(x)$ is large enough that a detector can be trained, they are limited in that they cannot improve the adversarial robustness. In this study, we extend the idea of adversarial detector and show that a light auxiliary network can improve the adversarial robustness. 
To the best of our knowledge, this is the first study to propose a purifier with a BCE loss over clean and adversarial examples. The design of the detector, however, is closely related to information theoretic principles where representations of two different layers are utilized. The training is also different in that AVmixup is used for a specific reason.
%
% [TODO: consider listing a few more papers? we have only two..]
\vspace*{-.2cm}
\subsection{Information maximization principles}
\label{sec:background:infomax}
Following the principle of maximum information preservation in \cite{linsker1988self} and the information maximization approach in \cite{bell1995information}, \citet{hjelm2018learning} demonstrated that unsupervised learning of representations is possible by maximizing mutual information between an input and the output of a deep neural network. 
For the main classifier network in our study, we consider a lower layer's representation $h_{low}(x)$ and a higher layer's representation $h_{high}(x)$ for a given input image $x$. 
Subsequently, the information maximization principles state that there should be a strong information theoretic relationship between $h_{low}(x)$ and $h_{high}(x)$. The relationship, however, is likely to be weaker or different for adversarial examples because the network has not seen adversarial examples during training. With this motivation, we select two layers from the main classification network and pass their representations $h_{low}(x)$ and $h_{high}(x)$ to the auxiliary network. 
According to the information maximization principles, it would be natural to maximize the mutual information between $h_{low}(x)$ and $h_{high}(x)$. Unfortunately, the precise estimation of mutual information is known to be difficult~\cite{mcallester2020formal,Song2020Understanding}. A known workaround for this problem is to evaluate BCE loss or Jensen-Shannon divergence between the positive example pairs of $(h_{low}(x_i), h_{high}(x_i))$ and the negative example pairs of $(h_{low}(x_i), h_{high}(x_j))$~\cite{hjelm2018learning, brakel2017learning, velickovic2018deep, ravanelli2018learning}, known as contrastive learning~\cite{hadsell2006dimensionality}. In our AID-Purifier, we also use a BCE loss but we discriminate between $(h_{low}(x_{adv}), h_{high}(x_{adv}))$ and $(h_{low}(x_{clean}), h_{high}(x_{clean}))$ instead. This can be a natural choice for adversarial defense, because the information theoretic relationship between $h_{low}(x)$ and $h_{high}(x)$ should be different for clean examples and adversarial examples. In particular, the perturbation of features induced by $x_{adv}$ increases gradually as it passes through the network~\cite{guo2017countering,liao2018defense,xie2019feature}. 
The auxiliary network is denoted as $D(h_{low}(x), h_{high}(x))$. 

\vspace*{-.2cm}
\subsection{AVmixup}
\label{sec:backgroud:AVmixup}
\citet{zhang2018mixup} proposed mixup that is a data augmentation scheme with linearly interpolated training examples for regularizing deep networks. Mixup can be considered as a derivative of label smoothing~\cite{szegedy2016rethinking}. As a variant of the mixup, \citet{lee2020adversarial} proposed AVmixup for performing data augmentation of adversarial examples. 
In AVmixup, a virtual example called an Adversarial Vertex (AV) is first defined. For a given pair of a clean example and the corresponding adversarial example, their AV lies in the same direction as the adversarial example, but $\gamma$ times farther away from the clean example. By controlling $\gamma$, the effect of data augmentation can be controlled. Once an AV example is defined, AVmixup extends the training distribution via linear interpolations of the clean example and the corresponding AV example. 
While AVmixup was shown to be effective for the adversarial training of the main classification network $C(x)$, we apply AVmixup to train the auxiliary discriminator network $D(h_{low}(x), h_{high}(x))$. This data augmentation with linear interpolation plays a pivotal role in training AID-Purifier. As a basic iterative procedure is applied at the inference time for purification, the discriminator needs to learn how to purify not only a strong adversarial example but also a weak adversarial example. Ideally, we would like the discriminator to learn a continuous path for purifying an adversarial example with an iterative procedure.




==> TEX/994_result_backup.tex <==
\section{Experiments}
\label{sec:experiment}
It is certainly possible to use a purifier as a stand-alone defense, but some of the purifiers can be also used as an add-on defense for boosting the performance of another adversarial defense. In this section, we investigate the performance of AID-Purifier as a stand-alone defense and as an add-on defense. 

\paragraph{Implementation details:} 
We perform the experiments over four datasets - SVHN~\cite{netzer2011reading}, CIFAR-10~\cite{krizhevsky2009learning}, CIFAR-100~\cite{krizhevsky2009learning}, and TinyImageNet~\cite{le2015tiny}. 
%
As in other studies~\cite{madry2017towards, pmlr-v97-zhang19p}, we use a 10-widen Wide-ResNet-34 \cite{zagoruyko2016wide} as the main classification network $C(x)$. 
%
For the white-box adversarial attack, we consider PGD~\cite{madry2017towards}, C\&W~\cite{carlini2017towards}, DeepFool (DF)~\cite{moosavi2016deepfool}, and MIM~\cite{dong2018boosting}. 
%
Additional details on network architecture and hyperparameters of AID-Purifier and benchmark models can be found in Appendix~\ref{sec:exp_detail_appendix}. Hyperparameters of the white-box attacks can be also found in Appendix~\ref{sec:exp_detail_appendix}. 



 \vspace*{-.2cm}
\subsection{Comparison with other adversarial purifiers} 
\label{sec:experiment_purification}
Among the four adversarial purifiers in Figure~\ref{fig:purification_concept}, we exclude MagNet~\cite{meng2017magnet} (a denoising purifier) and SOAP~\cite{shi2021online} (a SSL-based purifier) from our experiments. 
As explained in Section~\ref{sec:introduction}, MagNet is vulnerable to auxiliary-aware attack and SOAP cannot be used as an add-on. Thus, we only focus on Defense-GAN~\cite{samangouei2018defensegan} and PixelDefend~\cite{song2018pixeldefend}. As with AID-Purifier, both are robust against auxiliary-aware attack and can be used as an add-on. For the baseline adversarial training models of add-on experiments, we use Madry~\cite{madry2017towards}, Zhang~\cite{pmlr-v97-zhang19p}, and  Lee~\cite{lee2020adversarial} as the most representative set of defense models.

\vspace*{-.3cm}
\paragraph{Robust accuracy:} The robust accuracy results for SVHN are shown in Table~\ref{tab:comparison_purification}. Defense-GAN performs well as a stand-alone, but its performance as an add-on is inferior to the other purifiers. In fact, as an add-on, it usually undermines the baseline performance for complex datasets as shown in Appendix~\ref{sec:stand-alone_add-on_appendix}. For this reason, Defense-GAN is not investigated any further in Subsection~\ref{sec:experiment_non_purification}.  
 
\begin{table}[!t]
\vspace*{-.4cm}
\caption{Robust accuracy: stand-alone and add-on performances of adversarial purifiers are shown for the \textit{worst} white-box attack. SVHN dataset is evaluated below, and the results for other datasets can be found in Appendix~\ref{sec:stand-alone_add-on_appendix}.}
\vspace*{-.4cm}
\begin{center}
\resizebox{1\columnwidth}{!}{
\begin{tabular}{lrrrr}
\toprule
& \multicolumn{1}{c}{Stand-alone} & \multicolumn{3}{c}{Add-on} \\
\cmidrule(r){2-2} \cmidrule(r){3-5}
                 & \multicolumn{1}{l}{Natural training} & \multicolumn{1}{l}{Madry} & \multicolumn{1}{l}{Zhang}& \multicolumn{1}{l}{Lee} \\
                %  \cmidrule(r){1-1}\cmidrule(r){2-2}\cmidrule(r){3-3}\cmidrule(r){4-4}\cmidrule(r){5-5}
\midrule
No purification & 0.01 & 22.63 & 36.72 & 46.17 \\
Defense-GAN      & 41.89 & 28.42 & 38.60 & 43.42 \\
PixelDefend      & 23.34 & 52.83 & 55.42 & 64.14 \\
\textbf{AID-Purifier (Ours)}     & 29.10 & 49.85 & 44.76 & 62.70 \\   
PixelDefend + \textbf{AID-Purifier (Ours)} & \textbf{42.67} & \textbf{64.35} & \textbf{56.68} & \textbf{65.61} \\   
\bottomrule
\end{tabular}
}
\end{center}
\label{tab:comparison_purification}
\vspace*{-.2cm}
\end{table}

\begin{table}[t]
\vspace*{-.4cm}
\caption{Computational load: Purification time (i.e., inference time) and training time of the adversarial purifiers. Purification time was measured with batch size one. The reported values were measured with a single RTX2080ti, except for the training time of PixelDefend's TinyImageNet that was measured with four RTX2080ti's due to the memory requirement.}
\label{tab:computing_time}
\resizebox{1\columnwidth}{!}{
\begin{tabular}{lrrrrrrrr}
\toprule
& \multicolumn{2}{c}{SVHN} & \multicolumn{2}{c}{CIFAR-10} & \multicolumn{2}{c}{CIFAR-100} & \multicolumn{2}{c}{TinyImageNet} \\ 
 \cmidrule(r){2-3} \cmidrule(r){4-5} \cmidrule(r){6-7} \cmidrule(r){8-9} 
& \multicolumn{1}{c}{Purification} & \multicolumn{1}{c}{Training} 
& \multicolumn{1}{c}{Purification} & \multicolumn{1}{c}{Training} &
\multicolumn{1}{c}{Purification} & \multicolumn{1}{c}{Training} &
\multicolumn{1}{c}{Purification} & \multicolumn{1}{c}{Training} \\
& \multicolumn{1}{c}{time} & \multicolumn{1}{c}{time} &
\multicolumn{1}{c}{time} & \multicolumn{1}{c}{time} &
\multicolumn{1}{c}{time} & \multicolumn{1}{c}{time} &
\multicolumn{1}{c}{time} & \multicolumn{1}{c}{time} \\
& \multicolumn{1}{c}{(sec/img)} & \multicolumn{1}{c}{(min)} &
\multicolumn{1}{c}{(sec/img)} & \multicolumn{1}{c}{(min)} &
\multicolumn{1}{c}{(sec/img)} & \multicolumn{1}{c}{(min)} &
\multicolumn{1}{c}{(sec/img)} & \multicolumn{1}{c}{(min)} \\
\cmidrule(r){1-1} \cmidrule(r){2-3} \cmidrule(r){4-5} \cmidrule(r){6-7} \cmidrule(r){8-9} 
Defense-GAN & 0.14 & 205 & 0.13 & 197 & 0.14 & 198 & 0.31 & 1385 \\
PixelDefend & 41.97 & 1185 & 40.54 & 1056 & 40.96 & 1056 & 166.31 & \textit{5131} \\
\textbf{AID-Purifier (Ours)} & 0.59 & 23 & 0.59 & 15 & 0.59 & 16 & 0.60 & 147 \\
% PixelDefend + \textbf{AID-Purifier (Ours)} &                         1208 &  &                        1071  &   &                        1072 &   &                       5278 \\ 
\bottomrule
\end{tabular}
}
\vspace*{-.4cm}
\end{table}

Both of PixelDefend and AID-Purifier show positive improvements as a stand-along defense, but the performance is far from being impressive. When both are utilized together, however, they achieve $42.67\%$ of robust accuracy that is better than Madry or Zhang as a stand-alone. As an add-on, each of PixelDefend and AID-Purifier creates large improvements over all three adversarial training models. In fact, the best performance is achieved when both are utilized together. This synergy is due to the diversity between PixelDefend and AID-Purifier, and the diversity will be discussed further in Section~\ref{sec:discussions}. In Table~\ref{tab:comparison_purification}, PixelDefend tends to perform better than AID-Purifier as an individual model. An exhaustive comparison will be provided in Subsection~\ref{sec:experiment_non_purification}. 

Finally, we note that the stand-alone performances for complex datasets tend to be marginal for all of PixelDefend, AID-Purifier, and PixelDefend$+$AID-Purifier. Therefore, the purifiers will be more valuable as an add-on as long as they can consistently improve the baseline defense models of Madry, Zhang, and Lee. This is exactly what we will show in Subsection~\ref{sec:experiment_non_purification}.


\vspace*{-.3cm}
\paragraph{Computational load:} For a high-throughput application such as an API service or a real-time object detection by an autonomous vehicle, it can be critical for an adversarial defense to have a minimum impact on the inference time. Training time is also important as explained in ~\cite{NEURIPS2019_7503cfac, Wong2020Fast}. For a defense based on an adversarial training, the increase in training time is generally known to be large but the increase in inference time is negligible or zero. For a defense based on an adversarial purification, however, the increase in inference time (i.e., purification time) can be significant. 

We have measured the purification time and training time of the purifiers, and the results are shown in Table~\ref{tab:computing_time}. For the purification time, both defense-GAN and AID-Purifier perform well but PixelDefend is up to 277 times slower than AID-Purifier. This is due to the pixel-wise operation of PixelDefend, and the slow speed can be a critical limitation for certain applications. For the training time, AID-Purifier is definitely faster than the other two purifiers. Training of AID-Purifier is fast because a binary cross-entropy loss is used and because the training is typically completed within one epoch. The result includes the time for generating adversarial examples. The other two purifiers are trained as generative models and the training is slow. In fact, training of a generative model can be tricky in general.  


\vspace*{-.2cm}
\subsection{Boosting performance as an add-on} 
\label{sec:experiment_non_purification}
As a deep dive, we provide add-on experiment results for PixelDefend and AID-Purifier in Table~\ref{tab:comparison_w_adv_training}. Exhaustive results are provided in Appendix~\ref{sec:appendix_experiment_non_purification}.
The most important finding is that each of the two adversarial purifiers provides a positive enhancement for almost any individual combination of dataset and attack method. 
For the worst performance column, which can be considered as the overall conclusion for each dataset, PixelDefend$+$AID-Purifier achieves 42.11\% (46.17 to 65.61), 3.43\% (55.32 to 57.22), 13.75\% (28.51 to 32.43), and 13.12\% (26.91 to 30.44) of performance boosting for SVHN, CIFAR-10, CIFAR-100, and TinyImageNet, respectively. 
%
AID-Purifier alone, which requires only a light increase in the computational load, also achieves 35.80\% (46.17 to 62.70), 1.32\% (55.32 to 56.05), 7.26\% (28.51 to 30.58), and 14.49\% (26.91 to 30.81) of performance boosting.


\begin{table}[!t]
\vspace*{-0.2cm}
\caption{Robust accuracy: Experiment results of PixelDefend and AID-Purifier are shown for the \textit{worst} white-box attack. 
% SVHN, CIFAR-10, CIFAR-100, and TinyImageNet datasets are evaluated. 
As an add-on, each of PixelDefend and AID-Purifier provides a positive improvement for almost any individual combination of dataset and attack method. By inspecting the worst performance column of each dataset, it can be observed that PixelDefend$+$AID-Purifier achieves the best performance for three datasets and AID-Purifier achieves the best performance for TinyImageNet, which is the most complex dataset in our experiments.}
\label{tab:comparison_w_adv_training}
\resizebox{1\columnwidth}{!}{
\begin{tabular}{lrrrrr}
\toprule
Method & \multicolumn{1}{c}{SVHN} & \multicolumn{1}{c}{CIFAR-10} & \multicolumn{1}{c}{CIFAR-100} & \multicolumn{1}{c}{TinyImageNet}\\
% \cmidrule(r){1-1} \cmidrule(r){2-7} \cmidrule(r){8-13}
% Method & \multicolumn{1}{c}{Worst} & \multicolumn{1}{c}{Worst} & \multicolumn{1}{c}{Worst} & \multicolumn{1}{c}{Worst} \\
\midrule
% \cmidrule(r){1-1} \cmidrule(r){2-6} \cmidrule(r){7-7} \cmidrule(r){8-12} \cmidrule(r){13-13}
Natural training & 0.01 & 0.00 & 0.02 & 0.00\\
Madry~\cite{madry2017towards} & 22.63 & 51.64 & 25.42 & 20.79 \\
Zhang~\cite{pmlr-v97-zhang19p} & 36.72 & \underline{55.32} & \underline{28.51} & 20.96\\
Lee~\cite{lee2020adversarial} & \underline{46.17} & 46.44 & 27.35 & \underline{26.91} \\

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \cmidrule(r){1-1} \cmidrule(r){2-6} \cmidrule(r){7-7} \cmidrule(r){8-12} \cmidrule(r){13-13}
\midrule
Natural training + PixelDefend & 23.34 & 29.41 & 20.78 & 0.66\\
Madry~\cite{madry2017towards} + PixelDefend  & 52.83 & 54.75 & 27.34 & 21.81\\
Zhang~\cite{pmlr-v97-zhang19p} + PixelDefend & 55.42 & \underline{56.68} & 30.61 & 24.21\\
Lee~\cite{lee2020adversarial} + PixelDefend & \underline{64.14} & 51.83 & \underline{30.82} & \underline{29.81} \\ 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \cmidrule(r){1-1} \cmidrule(r){2-6} \cmidrule(r){7-7} \cmidrule(r){8-12} \cmidrule(r){13-13}
\midrule
Natural training + \textbf{AID-Purifier (Ours)} & 29.10 & 1.35 & 1.72 & 0.52\\
Madry~\cite{madry2017towards} + \textbf{AID-Purifier (Ours)}  & 49.85 & 52.65 & 27.71 & 21.67\\
Zhang~\cite{pmlr-v97-zhang19p} + \textbf{AID-Purifier (Ours)}  & 44.76 & \underline{56.05} & \underline{30.58} & 23.98\\
Lee~\cite{lee2020adversarial} + \textbf{AID-Purifier (Ours)} & \underline{62.70} & 49.13 & 29.35 & \underline{\textbf{30.81}}\\ 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \cmidrule(r){1-1} \cmidrule(r){2-6} \cmidrule(r){7-7} \cmidrule(r){8-12} \cmidrule(r){13-13}
\midrule
Natural training + PixelDefend + \textbf{AID-Purifier (Ours)}  & 42.67 & 35.82 & 23.89 & 2.66\\
\citet{madry2017towards} + PixelDefend + \textbf{AID-Purifier (Ours)}  & 64.35 & 55.07 & 28.70 & 21.85\\
\citet{pmlr-v97-zhang19p} + PixelDefend + \textbf{AID-Purifier (Ours)}  & 56.68 & \underline{\textbf{57.22}} & 30.99 & 24.34\\
\citet{lee2020adversarial} + PixelDefend + \textbf{AID-Purifier (Ours)} & \underline{\textbf{65.61}} & 53.33 & \underline{\textbf{32.43}} & \underline{30.44}\\
\bottomrule
\end{tabular}
}
\vspace*{-0.7cm}
\end{table}






\vspace*{-.2cm}
\subsection{Performance against auxiliary-aware attack and black-box attack} 
\label{sec:other_attacks}

\citet{shi2021online} devised an auxiliary-aware attack that is a complete white-box attack where both of the main classification network and the auxiliary network are known to the attacker. As shown in Figure~\ref{fig:aux} in Appendix~\ref{sec:aux_attack_appendix}, the auxiliary-aware attack completely fails on AID-Purifier because emphasizing auxiliary network attack weakens the strength of main network attack.

\citet{papernot2017practical} devised a black-box attack that generates adversarial images without any knowledge on the main classifier. As shown in Table~\ref{table:black_box} in Appendix~\ref{sec:blackbox_attack_appendix}, the black-box attack is not very effective to  AID-Purifier. % where AID-Purifier achieves at least 84.16\% of accuracy for CIFAR-10. 



==> TEX/9950_discussion_backup.tex <==
\section{Discussions}
\label{sec:discussions}

\subsection{Ablation study}
\label{sec:ablation tests}
To verify that the key features of AID-Purifier are effective, we have performed ablation tests. The results are shown in Table~\ref{tab:ablation}. All of the three key features are helpful for enhancing the performance of AID-Purifier, where the choice of training target and the choice of data augmentation scheme are crucial for AID-Purifier's performance.  



\begin{table}[b]
\vspace*{-0.7cm}
\centering
\caption{Ablation test results over the key features of AID-Purifier: The evaluations are over Madry, SVHN, and PGD. The baseline performance of Madry without any add-on is 38.17\%. 
(a) Number of intermediate layers connected from $C(x)$ to the discriminator. 
(b) Training targets.
(c) Data augmentation method for training.}
\label{tab:ablation}
\resizebox{1\columnwidth}{!}{
\begin{tabular}{ccc}
\begin{tabular}{p{2.1cm}p{2cm}}
\\
\\
\toprule
\multicolumn{1}{c}{Number of $h(x)$} & \multicolumn{1}{r}{Accuracy (\%)} \\
\midrule
\multicolumn{1}{c}{1} & \multicolumn{1}{r}{48.93} \\
\multicolumn{1}{c}{2} & \multicolumn{1}{r}{\textbf{49.85}}  \\
\bottomrule
\end{tabular}
&
\begin{tabular}{p{2.1cm}p{2cm}}
\\
\\
\toprule
\multicolumn{1}{c}{Targets} & \multicolumn{1}{r}{Accuracy (\%)} \\ \midrule
Contrastive & \multicolumn{1}{r}{44.87} \\
Clean vs. adv. & \multicolumn{1}{r}{\textbf{49.85}}  \\ \bottomrule
\end{tabular}
&
\begin{tabular}{p{2.1cm}p{2cm}}
 
\toprule
\multicolumn{1}{c}{Augmentation}       & \multicolumn{1}{r}{Accuracy (\%)} \\ \midrule
None             & \multicolumn{1}{r}{46.02}     \\
AV               & \multicolumn{1}{r}{47.73}     \\
Mixup            & \multicolumn{1}{r}{48.49}     \\
AVmixup          & \multicolumn{1}{r}{\textbf{49.85}} \\ \bottomrule
\end{tabular}
\\
\\
(a) Number of $h(x)$ & (b) Training targets & (c) Data augmentation \\
\end{tabular}
}
\end{table}



\subsection{Adversarial purifiers as performance boosters}
\label{sec:booster}
In Section~\ref{sec:experiment_non_purification}, it was shown that AID-Purifier and PixelDefend can be highly useful as add-on defenders that can be used in addition to a high-performance defender such as Madry, Zhang, and Lee. When the computational overhead of purification is of concern, AID-Purifier alone can be used as a computationally light add-on. When the computational overhead of purification is not of concern, both of AID-Purifier and PixelDefend can be used together for an extra improvement in robust accuracy. The extra improvement is due to the diversity between the two purifiers. PixelDefend's purification is based on the distribution $p_{data}(x)$ that is learned by PixelCNN. AID-Purifier's purification is based on the distributions $p_{clean}$ and $p_{adv}$ that are learned by the discriminator. While PixelDefend attempts to purify an example by pushing it to a high $p_{data}(x)$ region, AID-Purifier is more adventurous because it is willing to utilize out-of-distribution regions as well. The diversity between the two purifiers create a room for synergy. 

Considering the high performance of latest adversarially-trained models, it might be fair to assume that an adversarially-trained model should be always used as the base model while one or more purifiers could be used to boost its performance. To investigate if AID-Purifier can create a positive synergy with purifiers other than PixelDefend, we have carried out an extra experiment. In Appendix~\ref{sec:comparison_nrp}, NRP~\cite{naseer2020self} instead of PixelDefend is used to create a table in the same form as Table~\ref{tab:comparison_w_adv_training}. NRP is a type of adversarial purifier, that trains a conditional GAN to learn an optimal input processing function that enhances model robustness.
For NRP, the results in Table~\ref{tab:comparison_w_adv_training_appendix} of Appendix~\ref{sec:comparison_nrp} are similar to PixelDefend's results - AID-Purifier and NRP can create positive synergies. For the case of Defense-GAN, we have shown in Appendix~\ref{sec:stand-alone_add-on_appendix} that it can have negative effects for CIFAR-10, CIFAR-100, and TinyImageNet. In any case, we have tried using AID-Purifier together with Defense-GAN, and we have found that the loss by Defense-GAN can be mitigated by AID-Purifier as shown in Appendix~\ref{sec:comparison_dfgan}. 

Even though we have considered only adversarially-trained models as the base models to improve, the base model does not need to be limited in such a way. As long as a purifier is light in computation and attachable to frozen networks, it can be used as an add-on to boost \textit{any} adversarial defense network. For the case of PixelDefend and NRP, the results in Table~\ref{tab:comparison_w_adv_training} and Table~\ref{tab:comparison_w_adv_training_appendix} can be carefully examined to confirm that AID-Purifier can positively improve stand-alone defense of PixelDefend or NRP. This confirms that it is not necessary for an adversarially-trained network to be the base model, and a stand-along purifier can be the base model to be improved. PixelDefend and NRP, however, are also auxiliary purifiers and perhaps they should not be considered as a base model. In general, it remains as a future work to answer if adversarial purifiers should be always included as the last step add-on. 


\vspace*{-.2cm}
\subsection{Limitations and additional investigations}
\label{sec:limitation} 
In contrast to the mainstream purification methods, AID-Purifier does not aim to modify an adversarial image to a clean image. Our method allows $x_{pur}$ to be moved to out-of-distribution regions, and it can be confirmed from $x_{pur}$ in Figure~\ref{fig:our_method}. The image is a real example of $x_{pur}$ that was created by AID-Purifier. 

\citet{tramer2020adaptive} found that many combined defenses result in lower robustness than adversarial training alone, and a strong adaptive attack can be used to reveal the problem. In our study, we have performed auxiliary-aware attack as a strong adaptive attack and showed that the purification add-on is robust to the attack. Furthermore, we have investigated the influence of attack hyperparameters, attack epsilon, and the number of attack iterations for PGD attack as shown in Appendix~\ref{sec:sensitivity_appendix_att_hp}, and found that AID-Purifier can boost the performance for all the cases that were studied. Nonetheless, there might be other strong adaptive attacks that we might have missed to investigate.  

We additionally investigate the sensitivities of the attack method, the defense epsilon, and the number of iterations for training discriminator. The results can be found in Appendix~\ref{sec:sensitivity_appendix_att_for_D} and~\ref{sec:sensitivity_appendix_def_eps_iter}. 


% \subsection{Negative societal impacts}
% \label{sec:Negativesocietalimpacts} 
% Our study may increase the understanding of the attackers who aim to attack the deep learning systems. However, we believe our study will contribute to the knowledge of the research community and be used in positive directions. 

